Integrative Wrapping System for a Dual-Arm Humanoid Robot

Flexible object manipulation of paper and cloth is a major research challenge in robot manipulation. Although there have been efforts to develop hardware that enables specific actions and to realize a single action of paper folding using sim-to-real and learning, there have been few proposals for humanoid robots and systems that enable continuous, multi-step actions of flexible materials. Wrapping an object with paper and tape is more complex and diverse than traditional manipulation research due to the increased number of objects that need to be handled, as well as the three-dimensionality of the operation. In this research, necessary information is organized and coded based on the characteristics of each object handled in wrapping. We also generalize the hardware configuration, manipulation method, and recognition system that enable humanoid wrapping operations. The system will include manipulation with admittance control focusing on paper tension and state evaluation using point clouds to handle three-dimensional flexible objects. Finally, wrapping objects with different shapes is experimented with to show the generality and effectiveness of the proposed system.

==> src/acknowledge.tex <==
\section*{ACKNOWLEDGMENT}

The preferred spelling of the word acknowledgment in America is without an e after the g. Avoid the stilted expression, One of us (R. B. G.) thanks ...  Instead, try R. B. G. thanks. Put sponsor acknowledgments in the unnumbered footnote on the first page.

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



==> src/chap2_wrapping_character.tex <==
\section{chap2_wrapping_character}
手順が決まっており、前の手順の成否が直接次の手順に影響する


==> src/conclusion.tex <==
\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 


==> src/discussions.tex <==
\section{Discussions}
hoge


==> src/howto.tex <==
\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named Heading 1, Heading 2, Heading 3, and Heading 4 are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation Fig. 1, even at the beginning of a sentence.

\begin{table}[h]
  \caption{An Example of a Table}
  \label{table:example}
  \begin{center}
    \begin{tabular}{|c||c|}
      \hline
      One & Two\\
      \hline
      Three & Four\\
      \hline
    \end{tabular}
  \end{center}
\end{table}


\begin{figure}[thpb]
  \centering
  \includegraphics[width=\columnwidth]{nowprinting.eps}
  \caption{Inductance of oscillation winding on amorphous
    magnetic core versus DC bias magnetic field}
  \label{figure:label}
\end{figure}


Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity Magnetization, or Magnetization, M, not just M. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write Magnetization (A/m) or Magnetization {A[m(1)]}, not just A/m. Do not label axes with a ratio of quantities and units. For example, write Temperature (K), not Temperature/K.



==> src/math.tex <==
\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as 3.5-inch disk drive.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: Wb/m2 or webers per square meterﾓ, not webers/m2.  Spell out units when they appear in text: . . . a few henries, not . . . a few H.
\item Use a zero before decimal points: 0.25, not .25. Use cm3, not cc. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use (1), not Eq. (1) or equation (1), except at the beginning of a sentence: Equation (1) is . . .

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word data is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter o.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an inset, not an insert. The word alternatively is preferred to the word alternately (unless you really mean something that alternates).
\item Do not use the word essentially to mean approximately or effectively.
\item In your paper title, if the words that uses can accurately replace the word using, capitalize the u; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones affect and effect, complement and compliment, discreet and discrete, principal and principle.
\item Do not confuse imply and infer.
\item The prefix non is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the et in the Latin abbreviation et al..
\item The abbreviation i.e. means that is, and the abbreviation e.g. means for example.

\end{itemize}



==> src/procedure.tex <==
\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations


==> src/system_table.tex <==
\section{Characteristics of Wrapping Behavior and System Organization}
\begin{table*}[t]
  %% \caption{Targetの右側を包み込む包装における手順とそのそれぞれの手順において必要なハードウェア設計要件、認識、左右それぞれのハンドの制御・マニピュレーション方法}
  \caption{Procedure for wrapping the right side of the Target, including the necessary hardware design requirements, recognition, and control/manipulation methods for both left and right hands }
  \label{table:systemtable}
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c|c|l|l|l|l} \hline
      & Procedure & Hardware & Recognition & Rhand-Manipulation & Lhand-Manipulation \\ \hline \hline
      (i) & Preoperative Recognition & &
      \begin{tabular}{c}
        $T_{bbox} \gets f^{recog}_{1}(T_{pcl})$ \\ $W_{cbbox} \gets f^{recog}_{2}(W_{img}, W_{pcl})$ \\ $S_{cpm} \gets f^{recog}_{3}(S_{pcl})$
      \end{tabular}
      & & \\ \hline
      \multirow{2}{*}{(ii)} & \multirow{2}{*}{Lift Wrapper Upward} & \multirow{2}{*}{Hardness and Thinness of Nails} & & \multirow{2}{*}{$f^{ctrl}_{2}({W_{ab}})$}& \multirow{2}{*}{$f^{ctrl}_{1}(T_{abcd})$} \\ \cline{4-4}
      & & & $f^{recog}_{4}(W_{pcl})$ & & \\ \hline
      \multirow{4}{*}{(iii)} & \multirow{4}{*}{Cover} &
      \multirow{4}{*}{
      \begin{tabular}{c}
        Three-dimensional Shape \\ and Elasticity of the Fingers
      \end{tabular}}
      & & $f^{ctrl}_{3}(T_{ef}, (0, 0, -f))$} & \multirow{4}{*}{$\downarrow$} \\
        & & & & $f^{ctrl}_{3}(T_{ab}, (0, -f, 0))$ & \\
        & & & & $f^{ctrl}_{4}(Constraint = Target)$ & \\ \cline{4-4}
        & & & $W_{cbbox|abcd+} \gets f^{recog}_{5}(W_{pcl}, W_{cbbox})$ & &  \\ \hline
        \multirow{2}{*}{(iv)} & \multirow{2}{*}{Gripping Seal} & & & & \multirow{2}{*}{$f^{ctrl}_{5}(S_{cpm})$} \\ \cline{4-4}
      & & & $f^{ctrl}_{6}(S_{cpm})$ & & \\ \hline
      \multirow{3}{*}{(v)} & \multirow{3}{*}{
      \begin{tabular}{c}
        Securing Wrapper to Target \\ with Seal
      \end{tabular}}
      & & $W_{ab} \gets f^{recog}_{7}(W_{img}, W_{pcl}, T_{bbox}, W_{cbbox})$ & & \multirow{3}{*}{$f^{ctrl}_{4}(Constraint=Seal)$} \\ \cline{4-4}
      & & & $f^{recog}_{8}(S_{pcl}, T_{abcd})$ & & \\
      & & & $W_{cbbox|abcd+} \gets f^{recog}_{5}(W_{pcl}, W_{cbbox})$ & & \\ \hline
      \multirow{2}{*}{(vi)} & \multirow{2}{*}{
      \begin{tabular}{c}
        Evaluation of \\ Wrapping Condition
      \end{tabular}}
      & & $T_{bbox} \gets f^{recog}_{7}(T_{img}, T_{pcl}, T_{bbox})$ & & \\
      & & & $r \gets f^{recog}_{9}((T+W)_{pcl}, \vec{n_{abcd}}, \vec{n_{abfe}})$  & & \\ \hline
    \end{tabular}
  \end{adjustbox}
\end{table*}

\subsection{The characteristics of Wrapping}
\begin{enumerate}
%% \item 両手による操作の必要性
\end{enumerate}
\subsection{Target Object and System Configuration of Wrapping Actions}
%% ここでは包装動作で用いる対象物について、ロボットによる認識やマニピュレーションを行ううえでの特徴を整理する。それに基づき包装を行う手順とそのそれぞれの手順において必要なハードウェア設計要件、認識、左右それぞれのハンドの制御・マニピュレーション方法についてまとめる。

%% まず、包装動作で扱う対象物を整理する。一般的に包装は包装される対象物、それを包み込むもの、そして包み込むものを封じるものの3つを主に使って行う。本論文ではこの3つをそれぞれTarget、Wrapper、Sealと記号化する。

%% まずTargetについてであるが、Targetの特徴として、基本的に剛体であり、動作中に形状が変化しないことが挙げられる。本研究ではTargetを一般化し直方体状の箱を対象とする。Targetの中心点、向き、大きさの情報をbounding box(bbox)として取り扱い、bboxの値からわかるTarget直方体の頂点や辺とロボットとの位置関係を\figref{material-info}に表す。これ以降の説明において、例えばTargetの面や辺、大きさを$T_{abcd}$, $T_{ef}$, $T_{\overline{ab}}$のように示す。

%% 次にWrapperについてである。Wrapperは一般的に紙や布、プラスチックフィルムなどTargetを包み込める柔らかい素材を用いる。これらは薄い柔軟物体であり、包装動作中に曲げたり折ったりすることで形状が変化するため、高さのある形状が一定なbboxによる状態の記述は難しい。そこで、辺や動作途中に現れる折り目の線などの認識や色による点群の抽出による認識を行うこととなる。初期状態のWrapperを長方形とみなし、頂点の位置や向き、縦横の大きさ、色の情報を格納した情報を本研究では高さがない色付きbounding box(cbbox)とし、これによってWrapperを表す。cbboxとロボットとの位置関係を\figref{figure:material-info}に表す。

%% 最後にSealについてである。Sealは一般的に紙やプラスチックでできたテープやシールが使われる。Sealの特徴として、片面が粘着するという性質がある。また、丸められたりまとめられた状態からちぎったり破いたりして特定の大きさにしたりするため薄く柔らかく、加えて面積が小さい分張力も小さくなり、同様の素材でできたWrapperよりもさらに形状が不定となる。そのため、本研究では色付き点群による平均XYZ座標(CPM)でSealの状態を表すこととする。

%% 以上の各対象物の特徴を考慮に入れ、ロボットに対してTargetの右側を包み込む包装動作全体のシステムをまとめたものを\tabref{table:systemtable}にまとめる。

Here, we organize the characteristics of the objects used in the wrapping operation and summarize the requirements for hardware design, recognition, and control/manipulation methods for each step of wrapping based on it.

First, let's organize the objects involved in the wrapping operation. Generally, wrapping primarily involves three objects: the object being wrapped, the material wrapping it, and the material sealing it. In this paper, we symbolize these three as Target, Wrapper, and Seal, respectively.

Let's start with Target. The characteristic of Target is primarily its rigidity, meaning its shappe does not change during manipulation. In this study, we generalize Target to be a rectangular box. We handle information such as the center point, orientation, and size of the Target as a bounding box (bbox), and express the relationship between the vertices and edges of the Target rectangular prism and the robot using bbox values (\figref{material-info}). In the following explanations, for example, the faces or edges of the Target and their sizes will be represented as $T_{abcd}$, $T_{ef}$, $T_{\overline{ab}}$, respectively.

Next is Wrapper. Wrapper generally consists of soft materials such as paper, cloth, or plastic film that can wrap around the Target. These materials are thin and flexible, and their shape changes during the wrapping operation, making it difficult to describe their state using a fixed-height bbox. Therefore, recognition based on features like edges or crease lines appearing during the operation and extraction of point clouds based on color become necessary. We consider the initial state of the Wrapper as a rectangle and define it as a height-less colored bounding box (cbbox), storing information such as vertex positions, orientation, size in width and length, and color. The relationship between cbbox and the robot is depicted in \figref{material-info}.

Finally, Seal. Seals are typically tapes or stickers made of paper or plastic, with one side being adhesive. They are thin and flexible, allowing them to be torn or cut to a specific size from a rolled or folded state. Due to their small size and low tension compared to materials like Wrapper, Seals have a more indefinite shape. Therefore, we represent the state of Seal using the Colorized Point Cloud Mean (CPM).

Considering the characteristics of each object above, we summarize the entire wrapping operation system that wraps the right side of the Target using the robot in \tabref{systemtable}.

\begin{figure}[tbtp]
  \centering
  \includegraphics[width=0.5\columnwidth]{material-info.pdf}
  %% \capttion{Target, Wrapper, Sealの各情報とロボットとの位置関係}
  \caption{Positional relationship between Target, Wrapper, Seal, and the robot.}
  \label{figure:material-info}
\end{figure}

